Inpaint Biases: A Pathway to Accurate and Unbiased Image Generation

This paper examines the limitations of advanced text-to-image models in accurately rendering unconventional concepts which are scarcely represented or absent in their training datasets. We identify how these limitations not only confine the creative potential of these models but also pose risks of reinforcing stereotypes. To address these challenges, we introduce the Inpaint Biases framework, which employs user-defined masks and inpainting techniques to enhance the accuracy of image generation, particularly for novel or inaccurately rendered objects. Through experimental validation, we demonstrate how this framework significantly improves the fidelity of generated images to the user's intent, thereby expanding the models' creative capabilities and mitigating the risk of perpetuating biases. Our study contributes to the advancement of text-to-image models as unbiased, versatile tools for creative expression.

==> sec/2_literature_review.tex <==
\section{Preliminary}
\subsection{Large Language Models (LLMs)}

Large Language Models (LLMs) such as GPT (Generative Pre-trained Transformer) excel in text understanding and generation, offering significant contributions beyond mere text production. Their training on extensive datasets enables nuanced language comprehension and coherent response generation. A key advancement is their use in creative fields, particularly in enhancing text-to-image applications. By refining prompts based on user intent, LLMs significantly improve the creativity and relevance of generated images, showcasing their pivotal role in innovative content creation.

\subsection{Segment Anything Model (SAM)}

The Segment Anything Model (SAM) signifies a paradigm shift in image segmentation technology, capable of creating high-quality object masks based on input prompts like points or boxes. It is adept at generating detailed and precise masks for every object within an image. SAM's contribution is particularly noteworthy in streamlining workflows for subsequent tasks such as inpainting or advanced editing, demonstrating its value across multiple sectors requiring meticulous image analysis.

\subsection{Image Inpainting Methods}

Image inpainting, a complex inverse problem in computer vision, aims to restore missing parts of images with realistic structures and textures. The field has significantly advanced with deep learning, offering state-of-the-art methods differentiated by various inpainting strategies, network designs, and loss functions. [2] introduces an innovative approach enabling mask-free image inpainting, which allows users to interactively remove and fill regions, leveraging foundational models like Segment Anything, state-of-the-art inpainters, and AIGC models. However, the exploration of inpainting techniques, particularly beyond the basic scope of editing images to correspond with new prompts, remains insufficiently addressed in current research. This paper focuses on leveraging inpainting methods not just to modify images for new concepts but to enhance the alignment of existing prompts, ensuring more precise and contextually relevant image restorations.
